Towards Graph Contrastive Learning: A Survey and Beyond

In recent years, deep learning on graphs has achieved remarkable success in various domains. However, the reliance on annotated graph data remains a significant bottleneck due to its prohibitive cost and time-intensive nature. To address this challenge, self-supervised learning (SSL) on graphs has gained increasing attention and has made significant progress. SSL enables machine learning models to produce informative representations from unlabeled graph data, reducing the reliance on expensive labeled data. While SSL on graphs has witnessed widespread adoption, one critical component, Graph Contrastive Learning (GCL), has not been thoroughly investigated in the existing literature. Thus, this survey aims to fill this gap by offering a dedicated survey on GCL. We provide a comprehensive overview of the fundamental principles of GCL, including data augmentation strategies, contrastive modes, and contrastive optimization objectives. Furthermore, we explore the extensions of GCL to other aspects of data-efficient graph learning, such as weakly supervised learning, transfer learning, and related scenarios. We also discuss practical applications spanning domains such as drug discovery, genomics analysis, recommender systems, and finally outline the challenges and potential future directions in this field.

==> 5_1_lqq.tex <==
\subsection{Graph Weakly Supervised Learning}
% Graph Weakly Supervised Learning (GWSL) aims at using semi or few labels to . GWSL 
In many real-world scenarios, obtaining labeled data can be expensive or impractical, making semi-supervised learning particularly valuable. In response, Graph Weakly Supervised Learning (GWSL) are proposed to deal with this issue. GWSL leverages both labeled and unlabeled data to improve model performance. By effectively utilizing unlabeled data, semi-supervised graph learning can enhance model generalization, scalability, and robustness, making it an essential technique in graph learning tasks \cite{kipf2016semi,yan2024inductive,fang2021spatial}.

Existing GWSL methods can be roughly divided into three categories, i.e., label-propagating-based, pseudo-labeling-based, and regularizing-based ones.

\subsubsection{Label-Propagating GWSL}
Label Propagation (LP) utilizes the connectivity between nodes in the graph to propagate labels from labeled nodes to unlabeled ones. Specifically, it iteratively updates node labels to be similar to their neighbors, thereby leveraging the graph structure to infer labels for unlabeled nodes. The process of LP-based GWSL can be formalized as:
\begin{equation}
\begin{aligned}
    W^{*}, A^{*} &=\arg\min_{W,A}\mathcal{L}_{\text{sup}}(f(X,A),\mathcal{Y}) + \alpha\mathcal{L}_{\text{LP}}(f(A)), \\
                &= \arg\min_{W}\frac{1}{|\Theta|}\sum_{v_a\in \Theta} J(\hat{y_a}^{\text{gnn}},y_a) +  \\ 
                &\quad \arg\min_{A}\frac{1}{|\Theta|}\sum_{v_a\in \Theta} J(\hat{y_a}^{\text{lp}},y_a),
\end{aligned}
\end{equation}
where $\mathcal{L}_{\text{sup}}$ denotes the typical weakly supervised objective, $\mathcal{L}_{\text{LP}}$ denotes the label-propagating constraint, $v_a\in \Theta$ denotes the set of nodes with given labels, $X$ and $A$ denote the adjacent matrix and edge weight matrix respectively. $\alpha$ is a balancing hyper-parameter. Note that the optimal edge weights $A^{*}$ share the same topology as original $A$, as we do not add or remove edges but only focus on learning their weights. Generally speaking, LP propagates node label information across the edges, while GNN propagates and transforms node feature information \cite{yan2024inductive,song2020deep}.
GCN \cite{kipf2016semi} is a classical representative label-propagating GWSL work. It adopts a simple but effective message-passing scheme to make full use of the simi-labels. GCN-LPA \cite{wang2021combining} proposes a unified framework to combine GNN and LP to learn proper edge weights for better message-passing aggregation. Furthermore, it first systematically explores the relationships between LPA and GCN in theory. FLPA \cite{traag2023large} designs a fast label propagation based on processing the neighborhood-recently-changed nodes for large-scale graph mining. Adaprop \cite{zhang2023adaprop} designs an adaptive propagation path in the message-passing scheme to ignore irrelevant entities in a knowledge graph. Compared with traditional hand-crafted ones, the adaptive propagation path captures crucial correlations among entities and queries. ProtoLP \cite{zhu2023transductive} designs a prototype-based label propagation scheme for better graph construction with kernel functions, which is proven to be effective in the scenario of semi-supervised and few-shot learning. 

\subsubsection{Pseudo-Labeling GWSL}
Pseudo-Labeling (PL) GWSL augments the training set by using pseudo-labels generated by the model on unlabeled data. In semi-supervised graph learning, Pseudo-Labeling can leverage information from labeled nodes to generate pseudo-labels, which are then utilized to train the model, thereby improving its performance. A popular approach to semi-supervised learning is to create a graph that connects examples in the training dataset and propagate known labels through the edges of the graph to label unlabeled examples. An example of this approach to semi-supervised learning is the label propagation algorithm for classification predictive modeling \cite{long2019hierarchical,long2024unveiling}. The process of PL-based GWSL can be defined as:
\begin{equation}
\begin{aligned}
    W^{*}, A^{*} &=\arg\min_{W,A}\mathcal{L}_{\text{sup}}(f(X,A),\mathcal{Y}) + \alpha\mathcal{L}_{\text{PL}}\left (f(\Tilde{X},\Tilde{A}),\Tilde{\mathcal{Y}}\right ),\\
                &= \arg\min_{W}\frac{1}{|\Theta|}\sum_{v_a\in \Theta} J(\hat{y_a}^{\text{gnn}},y_a) + \\ 
                &\quad \arg\min_{W,A}\frac{1}{|V|}\sum_{v_i}^{|V|} J(\hat{y_i}^{\text{pl}},y_i^{\text{pl}}),
\end{aligned}
\end{equation}
where $\Tilde{X}$ denotes the selected unsupervised graph data feature, such as topological structure and community clustering. $\mathcal{Y}$ denotes the pseudo label of the unlabeled graph property $\Tilde{X}$. GLNN \cite{gao2020exploring} is a robust semi-supervised GNN, which is based on structure-adaptive graph learning. It adapts the graph topology to specific task labels and the input data. GSKN \cite{long2021theoretically} and HGK-GNN \cite{long2021hgk} are two representative structural Pseudo-Labeling GWSL works, which adopt structural graph kernel to capture graph topological structures. \cite{chen2021topology} proposes a topology-imbalance learning for semi-supervised graph node classification. SimP-GCN \cite{jin2021node} designs a $k$-nearest-neighbor graph based on the node features to enhance the neighbor aggregation performance. GLA \cite{yue2022label} conducts contrastive learning between a graph and its augmented views to learn graph representation for semi-supervised graph learning. Yu et. al \cite{yu2023semi} conduct a confidence-discriminative GNN, aiming at mining the potential information of unlabeled data. Compared with Label-Propagating GWSL, Pseudo-Labeling methods expand the training set by generating pseudo-labels on unlabeled data. At the same time, Label Propagation propagates labels from labeled nodes to unlabeled nodes using the connectivity in the graph structure.

\subsubsection{Regularizing GWSL}
Regularizing GWSL improves model generalization by encouraging the model to produce similar outputs for similar inputs. Semi-supervised graph learning can be achieved by augmenting input data or utilizing self-supervised signals from the graph structure. Its goal is to make the model produce consistent outputs on unlabeled data, thereby enhancing model robustness and generalization capability \cite{fang2022polarized,long2020graph}.
\begin{equation}
\begin{aligned}
    W^{*}, A^{*} &=\arg\min_{W,A}\mathcal{L}_{\text{sup}}(f(X,A),\mathcal{Y}) + \alpha\mathcal{L}_{\text{reg}}, \\
                &= \arg\min_{W}\frac{1}{|\Theta|}\sum_{v_a\in \Theta} J(\hat{y_a}^{\text{gnn}},y_a) + \\ 
                &\quad \arg\min_{A}\frac{1}{|V|}\sum_{v_i}^{|V|} \sigma\left (X_i^T,(\hat{A}Z)_{i}^T\right ),
\end{aligned}
\end{equation}
where $\mathcal{L}_{\text{reg}}$ denotes the regularization constraint.
\begin{equation}
\begin{aligned}
    ||\hat{A}Z-Z||_F^2 &=||(D^{-1}A-I)Z||_F^2 \\
                      &=\sum_{v_i}^{|V|} ||\left (\frac{1}{d_i}\sum_{j\in \mathcal{N}(v_i)}z_j\right )-z_i||_2^2
\end{aligned}
\end{equation}
In recent years, typical regularizing GWSL works have been proposed. Concretely, GNN-HF \cite{zhu2021interpreting} proposes a node-centered P-reg constraint to provide new 
InfoGraph \cite{sun2020infograph} jointly optimizes a supervised and an unsupervised model. The unsupervised constraint is a regularizing objective, which is further maximized through the mutual information with the supervised one. 
KGNN \cite{ju2022kgnn} designs a posterior regularization constraint for mutually enhancing semi-supervised mutuality between GNN and structural graph kernels under an EM-based framework. SizeShiftReg \cite{buffelli2022sizeshiftreg} comes up with a regularization objective for simulating a shift in the size of the training graphs using coarsening techniques and enforcing the model to be robust to such a shift. FASTRAIN-GNN \cite{nagarajan2023fastrain} designs a dynamic regularizer for overcoming the GNN layer effects and reducing the negative effects of incorrect simi-labels, which further significantly improves the quality of pseudolabels. IfMixup \cite{guo2023interpolating} leverages an effective visual regularizer \cite{zhang2017mixup}, to directly mix up input graph pairs in the learning process of GNNs.
